SignCRF: Scalable Channel-agnostic Data-driven Radio Authentication System

Radio Frequency Fingerprinting through Deep Learning (RFFDL) is a data-driven IoT authentication technique that leverages the unique hardware-level manufacturing imperfections associated with a particular device to recognize (fingerprint) the device based on variations introduced in the transmitted waveform. The proposed SignCRF is a scalable, channel-agnostic, data-driven radio authentication platform with unmatched precision in fingerprinting wireless devices based on their unique manufacturing impairments and independent of the dynamic channel irregularities caused by mobility. SignCRF consists of (i) a baseline classifier finely trained to authenticate devices with high accuracy and at scale; (ii) an environment translator carefully designed and trained to remove the dynamic channel impact from RF signals while maintaining the radio's specific signature; (iii) a Max-Rule module that selects the highest precision authentication technique between the baseline classifier and the environment translator per radio. We design, train, and validate the performance of SignCRF for multiple technologies in dynamic environments and at scale (100 LoRa and 20 WiFi devices). We demonstrate that SignCRF significantly improves the RFFDL performance by achieving as high as 5x and 8x improvement in correct authentication of WiFi and LoRa devices when compared to the state-of-the-art, respectively.

==> Figures/100_lora_.tex <==
\usetikzlibrary{patterns}
\pgfplotsset{width=10cm, height=5cm}

\pgfplotsset{
    compat=1.3,
    % define your own legend style here
    my ybar legend/.style={
        legend image code/.code={
            \draw [##1] (0cm,-0.6ex) rectangle +(3em,1.5ex);
        },
    },
}

\pgfplotscreateplotcyclelist{line_shape}{%
solid, every mark/.append style={solid, fill=red}, mark=diamond*\\%
dotted, every mark/.append style={solid,  fill=gray}, mark=square*\\%
densely dotted, every mark/.append style={solid, fill=gray}, mark=otimes*\\%
loosely dotted, every mark/.append style={solid, fill=gray}, mark=triangle*\\%
dashed, every mark/.append style={solid, fill=gray},mark=halfdiamond*\\%
loosely dashed, every mark/.append style={solid, fill=gray},mark=*\\%
densely dashed, every mark/.append style={solid, fill=gray},mark=square*\\%
dashdotted, every mark/.append style={solid, fill=gray},mark=otimes*\\%
dashdotdotted, every mark/.append style={solid},mark=star\\%
densely dashdotted,every mark/.append style={solid, fill=gray},mark=diamond*\\%
}

\begin{tikzpicture}
% \selectcolormodel{gray}
\begin{axis}[
cycle list name = line_shape,
ylabel style={align=center}, 
ylabel={LoRa TTOD\\ 100 radios.},
xlabel={Epochs},
xticklabels={0, 50, 100, 200},
xtick={0, 50, 100, 200},
legend style={at={(0.5,-0.3)},
anchor=north,legend columns=3},
% xtick=data,
mark size=2.5pt,
xmin =0,
xmax = 205,
% height=8cm,
width=8cm,
grid=major,
]
\addplot coordinates { (0, 0.06 ) (50, 0.20 )  (100, 0.30) (200, 0.37 ) };



% \legend{$100 LoRa TTOD performance$}
\end{axis}
\end{tikzpicture}



==> Figures/mix_days_wifi_5radios.tex <==
\usetikzlibrary{patterns}
\pgfplotsset{width=10cm, height=5cm}

\pgfplotsset{
    compat=1.3,
    % define your own legend style here
    my ybar legend/.style={
        legend image code/.code={
            \draw [##1] (0cm,-0.6ex) rectangle +(3em,1.5ex);
        },
    },
}

\pgfplotscreateplotcyclelist{line_shape}{%
solid, every mark/.append style={solid, fill=red}, mark=diamond*\\%
dotted, every mark/.append style={solid,  fill=gray}, mark=square*\\%
densely dotted, every mark/.append style={solid, fill=gray}, mark=otimes*\\%
loosely dotted, every mark/.append style={solid, fill=gray}, mark=triangle*\\%
dashed, every mark/.append style={solid, fill=gray},mark=halfdiamond*\\%
loosely dashed, every mark/.append style={solid, fill=gray},mark=*\\%
densely dashed, every mark/.append style={solid, fill=gray},mark=square*\\%
dashdotted, every mark/.append style={solid, fill=gray},mark=otimes*\\%
dashdotdotted, every mark/.append style={solid},mark=star\\%
densely dashdotted,every mark/.append style={solid, fill=gray},mark=diamond*\\%
}

\begin{tikzpicture}
% \selectcolormodel{gray}
\begin{axis}[
cycle list name = line_shape,
ylabel style={align=center}, 
ylabel={WiFi TTOD\\ 5 radio mdel},
xlabel={Number of mixed days},
xticklabels={1, 2, 3, 4, 5},
legend style={at={(0.5,-0.3)},
anchor=north,legend columns=3},
xtick=data,
mark size=2.5pt,
xmin =0,
xmax = 6,
% height=8cm,
width=8cm,
grid=major,
]
\addplot coordinates { (1, 0.17 ) (2, 0.13 )  (3, 0.15) (4, 0.16 ) (5, 0.24 )};

\addplot coordinates { (1, 0.2 ) (2, 0.18 )  (3, 0.2) (4, 0.18 ) (5, 0.19 )};
\addplot coordinates { (1, 0.26 ) (2, 0.24 )  (3, 0.26) (4, 0.19 ) (5, 0.23 )};

\legend{$Baseline\-1D$, $RNN\-LSTM$, $ResNet\1D$}
\end{axis}
\end{tikzpicture}



==> Figures/wifi_batch_comparison.tex <==
\usetikzlibrary{patterns}
\pgfplotsset{width=10cm, height=5cm}

\pgfplotsset{
    compat=1.3,
    % define your own legend style here
    my ybar legend/.style={
        legend image code/.code={
            \draw [##1] (0cm,-0.6ex) rectangle +(3em,1.5ex);
        },
    },
}

\pgfplotscreateplotcyclelist{line_shape}{%
solid, every mark/.append style={solid, fill=red}, mark=diamond*\\%
dotted, every mark/.append style={solid,  fill=gray}, mark=square*\\%
densely dotted, every mark/.append style={solid, fill=gray}, mark=otimes*\\%
loosely dotted, every mark/.append style={solid, fill=gray}, mark=triangle*\\%
dashed, every mark/.append style={solid, fill=gray},mark=halfdiamond*\\%
loosely dashed, every mark/.append style={solid, fill=gray},mark=*\\%
densely dashed, every mark/.append style={solid, fill=gray},mark=square*\\%
dashdotted, every mark/.append style={solid, fill=gray},mark=otimes*\\%
dashdotdotted, every mark/.append style={solid},mark=star\\%
densely dashdotted,every mark/.append style={solid, fill=gray},mark=diamond*\\%
}

\begin{tikzpicture}
% \selectcolormodel{gray}
\begin{axis}[
cycle list name = line_shape,
ylabel style={align=center}, 
ylabel={TTOD\%},
xlabel={Epochs},
xticklabels={10, 20, 30, 40, 50, 60, 70, 80, 90, 100},
legend style={at={(0.7,0.5)},
anchor=north,legend columns=1},
xtick=data,
mark size=2.5pt,
xmin =5,
xmax = 105,
% height=8cm,
width=8cm,
grid=major,
]
\addplot coordinates { (10, 0.37 )  (20, 0.36) (30, 0.39 ) (40, 0.38 ) (50, 0.38) (60, 0.38) (70, 0.388 ) (80, 0.36 ) (90, 0.36 ) (100, 0.36)};
%(300, 60) (Max Rule, 71)
\addplot coordinates {(10, 0.28 )  (20, 0.32 ) (30, 0.36) (40, 0.38 ) (50, 0.40) (60, 0.41) (70, 0.37 ) (80, 0.40 ) (90, 0.37 ) (100, 0.37)};
\addplot coordinates {(10, 0.24 )  (20, 0.32 ) (30, 0.34 ) (40, 0.31 ) (50, 0.36) (60, 0.38) (70, 0.35 ) (80, 0.39 ) (90, 0.37 ) (100, 0.37)};


\legend{$batch\_size-1$, $batch\_size-32$, $batch\_size-64$}
\end{axis}
\end{tikzpicture}



==> Figures/wifi_per_device_per_epoch.tex <==
\usetikzlibrary{patterns}
\pgfplotsset{width=10cm, height=5cm}

\pgfplotsset{
    compat=1.3,
    % define your own legend style here
    my ybar legend/.style={
        legend image code/.code={
            \draw [##1] (0cm,-0.6ex) rectangle +(3em,1.5ex);
        },
    },
}

\pgfplotscreateplotcyclelist{line_shape}{%
solid, every mark/.append style={solid, fill=red}, mark=diamond*\\%
dotted, every mark/.append style={solid,  fill=gray}, mark=square*\\%
densely dotted, every mark/.append style={solid, fill=gray}, mark=otimes*\\%
loosely dotted, every mark/.append style={solid, fill=gray}, mark=triangle*\\%
dashed, every mark/.append style={solid, fill=gray},mark=halfdiamond*\\%
loosely dashed, every mark/.append style={solid, fill=gray},mark=*\\%
densely dashed, every mark/.append style={solid, fill=gray},mark=square*\\%
dashdotted, every mark/.append style={solid, fill=gray},mark=otimes*\\%
dashdotdotted, every mark/.append style={solid},mark=star\\%
densely dashdotted,every mark/.append style={solid, fill=gray},mark=diamond*\\%
}

\begin{tikzpicture}
% \selectcolormodel{gray}
\begin{axis}[
cycle list name = line_shape,
ylabel style={align=center}, 
ylabel={TTOD \%},
xlabel={Epochs},
xticklabels={0, 10, 20, 30, 40, 50, 60, 70, 80, 90, 100},
legend style={at={(0.5,-0.3)},
anchor=north,legend columns=3},
xtick=data,
mark size=2.5pt,
xmin =0,
xmax = 105,
% height=8cm,
width=8cm,
grid=major,
]
\addplot coordinates { (0, 0.34 ) (10, 0.18 )  (20, 0.15) (30, 0.17 ) (40, 0.19 ) (50, 0.28) (60, 0.24) (70, 0.15 ) (80, 0.27) (90, 0.14 ) (100, 0.16)};

\addplot coordinates {(0, 0.17 ) (10, 0.29 )  (20, 0.42 ) (30, 0.50) (40, 0.50 ) (50, 0.46) (60, 0.51) (70, 0.48 ) (80, 0.51 ) (90, 0.48 ) (100, 0.50)};
\addplot coordinates {(0, 0.11 ) (10, 0.60 )  (20, 0.59 ) (30, 0.65 ) (40, 0.66 ) (50, 0.70) (60, 0.68) (70, 0.71 ) (80, 0.71 ) (90, 0.72 ) (100, 0.65)};
\addplot coordinates {(0, 0.03 ) (10, 0.09 )  (20, 0.09 ) (30, 0.15) (40, 0.15) (50, 0.12) (60, 0.17) (70, 0.12 ) (80, 0.15 ) (90, 0.10 ) (100, 0.16)};
\addplot coordinates {(0, 0.27 ) (10, 0.24 )  (20, 0.36) (30, 0.32) (40, 0.38) (50, 0.42) (60, 0.45) (70, 0.42 ) (80, 0.37 ) (90, 0.40 ) (100, 0.39)};


\legend{$radio-1$, $radio-2$, $radio-3$, $radio-4$, $radio-5$}
\end{axis}
\end{tikzpicture}



==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> myTiKz.tex <==
% tikz styles
\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=2cm, minimum height=0.5cm,text centered, draw=black]
\tikzstyle{io} = [trapezium, trapezium left angle=70, trapezium right angle=110, minimum width=3cm, minimum height=1cm, text centered, draw=black]
\tikzstyle{process} = [rectangle, minimum width=2cm, minimum height=0.5cm, text centered, draw=black, alignb=center]
\tikzstyle{decision} = [ellipse, minimum width=2cm, minimum height=1cm, text centered, draw=black]
\tikzstyle{arrow} = [thick,<->,>=stealth]
\tikzstyle{line} = [thick,>=stealth]
\tikzstyle{darrow} = [thick,<->,>=stealth,dashed]
\tikzstyle{sarrow} = [thick,->,>=stealth]
%\tikzstyle{larrow} = [line width=0.05mm,dashdotted,>=stealth]
\tikzstyle{larrow} = [line width=0.1mm,dashdotted,->,>=stealth]


\makeatletter
\def\grd@save@target#1{%
  \def\grd@target{#1}}
\def\grd@save@start#1{%
  \def\grd@start{#1}}
\tikzset{
  grid with coordinates/.style={
    to path={%
      \pgfextra{%
        \edef\grd@@target{(\tikztotarget)}%
        \tikz@scan@one@point\grd@save@target\grd@@target\relax
        \edef\grd@@start{(\tikztostart)}%
        \tikz@scan@one@point\grd@save@start\grd@@start\relax
        \draw[minor help lines] (\tikztostart) grid (\tikztotarget);
        \draw[major help lines] (\tikztostart) grid (\tikztotarget);
        \grd@start
        \pgfmathsetmacro{\grd@xa}{\the\pgf@x/1cm}
        \pgfmathsetmacro{\grd@ya}{\the\pgf@y/1cm}
        \grd@target
        \pgfmathsetmacro{\grd@xb}{\the\pgf@x/1cm}
        \pgfmathsetmacro{\grd@yb}{\the\pgf@y/1cm}
        \pgfmathsetmacro{\grd@xc}{\grd@xa + \pgfkeysvalueof{/tikz/grid with coordinates/major step x}}
        \pgfmathsetmacro{\grd@yc}{\grd@ya + \pgfkeysvalueof{/tikz/grid with coordinates/major step y}}
        \foreach \x in {\grd@xa,\grd@xc,...,\grd@xb}
        \node[anchor=north] at (\x,\grd@ya) {\pgfmathprintnumber{\x}};
        \foreach \y in {\grd@ya,\grd@yc,...,\grd@yb}
        \node[anchor=east] at (\grd@xa,\y) {\pgfmathprintnumber{\y}};
      }
    }
  },
  minor help lines/.style={
    help lines,
    gray,
    line cap =round,
    xstep=\pgfkeysvalueof{/tikz/grid with coordinates/minor step x},
    ystep=\pgfkeysvalueof{/tikz/grid with coordinates/minor step y}
  },
  major help lines/.style={
    help lines,
    line cap =round,
    line width=\pgfkeysvalueof{/tikz/grid with coordinates/major line width},
    xstep=\pgfkeysvalueof{/tikz/grid with coordinates/major step x},
    ystep=\pgfkeysvalueof{/tikz/grid with coordinates/major step y}
  },
  grid with coordinates/.cd,
  minor step x/.initial=.5,
  minor step y/.initial=.2,
  major step x/.initial=1,
  major step y/.initial=1,
  major line width/.initial=1pt,
}
\makeatother
